The LOCATA Challenge: Acoustic Source Localization and Tracking

The ability to localize and track acoustic events is a fundamental prerequisite for equipping machines with the ability to be aware of and engage with humans in their surrounding environment. However, in realistic scenarios, audio signals are adversely affected by reverberation, noise, interference, and periods of speech inactivity. In dynamic scenarios, where the sources and microphone platforms may be moving, the signals are additionally affected by variations in the source-sensor geometries. In practice, approaches to sound source localization and tracking are often impeded by missing estimates of active sources, estimation errors, as well as false estimates. The aim of the LOCAlization and TrAcking (LOCATA) Challenge is an open-access framework for the objective evaluation and benchmarking of broad classes of algorithms for sound source localization and tracking. This article provides a review of relevant localization and tracking algorithms and, within the context of the existing literature, a detailed evaluation and dissemination of the LOCATA submissions. The evaluation highlights achievements in the field, open challenges, and identifies potential future directions.

==> Content/Submissions.tex <==
% \begin{table*}[tb]
% \centering
% \caption{Summary of submitted localization and tracking frameworks. ID 5 is not included as details were not provided by the authors. The dash symbol, $-$, denotes subsystems that were not included in a specific submission.}
% \label{table:submissions}
% \begin{tabular}{|c||c|c||c||c|c||c|c||c|}
% \hline
% \multirow{2}{*}{ID} & \multirow{2}{*}{Details} & \multirow{2}{*}{Tasks} & \multirow{2}{*}{VAD} & \multicolumn{2}{|c||}{Localization} & \multicolumn{2}{|c||}{Tracking} & \multirow{2}{*}{Arrays} \\
% \cline{5-8}
% & & & & Algorithm & Section & Algorithm & Section & \\ \hline\hline
%  %
%  1 & \cite{Agcaer2018} & 1 & - & LDA classification & {\color{red}{Ref missing}} & - & - & Hearing Aids \\\hline
%  %
%  \multirow{4}{*}{2} & \multirow{4}{*}{\cite{Liu2018}} & \multirow{4}{*}{4} & \multirow{4}{*}{-} &  & &  & & Robot Head \\
%  & & & & \acs{MUSIC} & \ref{sec:literature_localization_multisource_subspace} & Particle PHD filter & \ref{sec:literature_tracking_multisource} & DICIT\\
%  & & & & & & + Particle Flow & & Hearing Aids \\
%  & & & & & & & & Eigenmike \\ \hline
%  %
%  3 & \cite{Qian2018} & 1,3,5 & - & GCC-PHAT & \ref{sec:literature_localization_singlesource_TDoA} & Particle filter
%  & \ref{sec:literature_tracking_singlesource} & DICIT \\\hline
%  %
%  \multirow{2}{*}{4} & \multirow{2}{*}{\cite{Li2018}} & \multirow{2}{*}{1-6} & \multirow{2}{*}{Variational EM} & Direct-path RTF + &
%   \ref{sec:literature_localization_singlesource_TDoA} & \multirow{2}{*}{Variational EM} & {\color{red}{Ref missing}} & \multirow{2}{*}{Robot Head}\\
%  &&&& GMM &&&& \\ \hline
%  %
%  \multirow{2}{*}{6} & \multirow{2}{*}{\cite{Lebarbechon2018}} & \multirow{2}{*}{1,3,5} & \multirow{2}{*}{-} & \multirow{2}{*}{SRP-PHAT} &
%  \multirow{2}{*}{\ref{sec:literature_localization_singlesource_TDoA}} & \multirow{2}{*}{-} & - & Eigenmike \\
%  & & & & & & & & Robot Head \\\hline
%  %
%  7 & \cite{Salvati2018a} & 1,3,5 & CPSD trace & SRP Beamformer &
%  \ref{sec:literature_localization_singlesource_direct} & Kalman filter &
%  \ref{sec:literature_tracking_singlesource} & DICIT \\\hline
%   %
%  8 & \cite{Mosgaard2018} & 1,3,5 & - & TDE using IPDs & \ref{sec:literature_localization_singlesource_binaural},
%  \ref{sec:literature_localization_singlesource_TDoA} &
%  Wrapped Kalman filter & \ref{sec:literature_tracking_singlesource} & Hearing Aids \\\hline
%  %
%  9 & \cite{Pak2018} & 1 & - & DNN & \ref{sec:literature_localization_multisource_deepLearning} & - & - & DICIT \\ \hline
%  %
%  \multirow{2}{*}{10} & \multirow{2}{*}{\cite{Kitic2018}} & \multirow{2}{*}{1-4} & \multirow{2}{*}{Noise PSD} & PIVs from &
%  \multirow{2}{*}{\ref{sec:literature_localization_singlesource_spherical}} & \multirow{2}{*}{Particle filter}
%  & \multirow{2}{*}{\ref{sec:literature_tracking_singlesource}} & \multirow{2}{*}{Eigenmike} \\
%  & & & & first-order ambisonics & & & & \\ \hline
%  %
%  11 & \cite{Madmoni2018} & 1,2 & - & DPD-Test + MUSIC &
%  \ref{sec:literature_localization_singlesource_direct} & - & - & Robot Head \\ \hline
%  %
%  \multirow{2}{*}{12} & \multirow{2}{*}{\cite{Madmoni2018}} & \multirow{2}{*}{1,2} & \multirow{2}{*}{-} & DPD-Test + &
%  \ref{sec:literature_localization_singlesource_direct} & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \multirow{2}{*}{Eigenmike} \\
%  & & & & MUSIC in SH-domain & \ref{sec:literature_localization_singlesource_spherical} & & & \\ \hline
%  %
%  13 & \cite{Nakadai2018} &  1,3 & Zero-crossing rate & MUSIC (SVD) & \ref{sec:literature_localization_singlesource_direct} & Kalman filter &
%  \ref{sec:literature_tracking_singlesource} & DICIT \\ \hline
%  %
%  14 & \cite{Nakadai2018} & 1,3 & Zero-crossing rate & MUSIC (GEVD) & \ref{sec:literature_localization_singlesource_direct} & Kalman filter &
%  \ref{sec:literature_tracking_singlesource} & DICIT \\ \hline
%  %
%  15 & \cite{Moore2018} & 1 & Baseline \cite{Sohn1999} & Subspace PIV & \ref{sec:literature_localization_singlesource_spherical} & - & - & Eigenmike \\ \hline
%  %
%  \multirow{2}{*}{16} & \multirow{2}{*}{\cite{Moore2018}} & \multirow{2}{*}{2} & \multirow{2}{*}{Baseline \cite{Sohn1999}} &
% Subspace PIV + & \multirow{2}{*}{\ref{sec:literature_localization_singlesource_spherical}} & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \multirow{2}{*}{Eigenmike} \\
%  & & & & Peak Picking & & & & \\ \hline
%  %
% \end{tabular}
% \end{table*}

% The following subsection summarizes the approaches submitted to the \ac{LOCATA} challenge, and grouped by approaches incorporating \begin{inparaenum}[a)] \item localization algorithms, i.e., \ac{DoA} estimators that provide instantaneous estimates of the source azimuth and, if applicable, elevation; \item tracking algorithms, incorporating spatio-temporal models of the source motion in order to predict future positional information, and to update the predictions by inferring new information as new sensor measurements become available. \end{inparaenum} An overview of the submissions is provided in \tabref{table:submissions}. Details of each approach are provided in the corresponding \ac{LOCATA} proceedings paper, provided in the references below.

% \subsection{Localization algorithms}
% \begin{description}[style=unboxed,leftmargin=0.25cm]
  % \item [ID 1 \cite{Agcaer2018}] proposes a classifier trained using binaural features from the hearing aids of the static single-source Task 1. Bandpass filters are applied to the signals captured by the four cardioid microphones of the hearing aid, where the passband range values of the filterbank are determined by model-based optimization. Amplitude modulation analysis is performed in each resulting time-frequency bin. Classification aims at distinguishing between 12 classes of potential source directions, where each class corresponds to a segment of $30^{\circ}$. Linear discriminant analysis (LDA) classification is performed using six classifiers, each shifted by $5^{\circ}$. The classifiers are trained using a \ac{HRTF} dataset and 18 speech signals of 10~s duration in each candidate direction and distorted by various noise types.
  % \item [ID 5] applies an implementation of the approach in \cite{Pavlidi2016} for the Eigenmike in all Tasks 1-6. Details are unknown since a challenge paper is not available.
  % \item [ID 6 \cite{Lebarbechon2018}] applies \ac{SRP}-\ac{PHAT} for the single-source Tasks 1, 3, and 5 using the robot head and the Eigenmike. For each microphone pair, the source angles are estimated from the signals in the \ac{STFT} domain over a search space in azimuth and elevation. The \ac{GCC}-\ac{PHAT} is evaluated for a resampled subset of the boresight estimates. A ``global'' angular spectrum is obtained by combining the \ac{GCC}-\ac{PHAT} across all time-frequency bins and microphone pairs within an overlapping sliding analysis window of 256-512~ms. Estimates of the source \acp{DoA} are extracted as the peaks in the global angular spectrum.
  % \item [ID 9 \cite{Pak2018}] proposes to use a \ac{DNN} regression model for localization of the source \ac{DoA} for the static single-source Task 1 using the signals of four microphones from the \ac{DICIT} array. The approach uses as features the phase differences between two channels, modified by the voice pitch. The \ac{DNN} is trained using a dataset of reverberant speech signals, simulated using the image-source method \cite{Allen1979} for different reverberation levels, and distorted by three noise types.
  % \item [ID 11 \cite{Madmoni2018}] utilizes the direct-path dominance test \cite{Nadiri2014} and \ac{MUSIC} for the robot head signals for static-source Tasks 1 and 2. A ``focusing'' process is applied to the microphone signals in the \ac{STFT} domain in order to remove the frequency-dependence \cite{Beit2018}. Frequency smoothing is applied to decorrelate coherent contributions due to the direct path signals and early reflections \cite{Nadiri2014}. The direct-path dominance test \cite{Nadiri2014} is used to identify time-frequency bins corresponding to the contribution of a single source only. The MUSIC pseudo-spectrum is evaluated for each bin that passes the test. Due to the static source-sensor geometry, the pseudo-spectra are combined over all time-frequency bins that passed the direct-path-dominance test. A single estimate per source is obtained by extracting the spectral peaks using $k$-means clustering. The estimates are extrapolated for all time frames.
  % \item [ID 12 \cite{Madmoni2018}] extends the approach detailed for Submission ID 11 to processing in the spherical harmonic domain of the Eigenmike signals for Tasks 1 and 2. The spherical harmonic transformation is applied to the \ac{STFT} signals, and the plane wave decomposition is evaluated. For each time-frequency bin, the local correlation matrix is evaluated. The \ac{DoA} estimates are obtained using the approach applied in ID 11.
%   \item [ID 15 \cite{Moore2018}] applies the subspace pseudo-intensity vector approach in \cite{Moore2017} to the Eigenmike data in the static-source Tasks 1. The spherical harmonic transformation is applied to the microphone signals in the \ac{STFT} domain. Mode strength compensation is applied to account for scattering off the rigid array baffle. The subspace pseudo-intensity vectors in each time-frequency bin are evaluated according to \cite{Moore2017}. Estimates of the source azimuth and inclination values are extracted from a histogram of the pseudo-intensity vector directions picking the largest peak.
%   \item [ID 16 \cite{Moore2018}] extends the approach in ID 15 for the static multi-source Task 2 by incorporating source counting. The 10 largest peaks are extracted from the smoothed histogram. A threshold is applied to the height of all peaks. The number of sources corresponds to the number of peaks remaining after thresholding, whilst the estimated source DOAs correspond to the peak locations.
% \end{description}

% \subsection{Tracking algorithms}
% \begin{description}[style=unboxed,leftmargin=0.25cm]
  % \item [ID 2 \cite{Liu2018}] utilizes \ac{DoA} estimates from \ac{MUSIC} as inputs to a \ac{PHD} filter \cite{Ristic2013,Mahler2007} and intensity particle flow \cite{Liu2017} for multi-source tracking in Task 4, evaluated for any of the four arrays. A particle filter implementation of the \ac{PHD} filter is used for tracking the multiple source positions, where the particles are predicted by prior importance sampling. Particle flow is used to move the particles from the prior to the posterior \ac{pdf}. The particle weights are evaluated using the modified particle states. Point estimates of the source positions are evaluated by $k$-means clustering. Each estimate is labelled with a track ID by assigning each estimate to the closest previous track.
  % \item [ID 3 \cite{Qian2018}] combines \ac{TDE} for localization with a particle filter for tracking using the \ac{DICIT} array for the single-source Tasks 1, 3 and 5. \ac{TDoA} estimates are obtained using \ac{GCC}-\ac{PHAT} for each frame of the \ac{STFT} signals. The \ac{TDoA} estimates are averaged to obtain the \ac{GCF} value \cite{Omologo1998} at each point in a discrete grid of candidate source positions. Localized source position estimates are obtained as the maximum value in the \ac{GCF}. Front-back ambiguity arising from the linear, symmetric geometry of the \ac{DICIT} array is addressed by hypothesis testing using the ratio of \acp{GCF} due to a source in the front versus a source in the back of the array. The localized estimates are used as the input of a particle filter using prior importance sampling \cite{Doucet2001}. The importance-weighted mean of the particles is used as the point estimate. Outliers during voice inactivity are removed by fixed-lag smoothing over a short time interval.
  % \item [ID 4 \cite{Li2018}] combines \ac{DoA} estimation using the direct-path \ac{RTF} approach in \cite{Li2016} with a variational \ac{EM} algorithm for multi-source tracking using the robot head for all Tasks. Recursive least-squares optimization is used to estimate the direct-path relative transfer function as a localization feature, associated with a single speaker at each time-frequency bin of the \ac{STFT} of the microphone signals. A complex \ac{GMM} is fitted to model the features. The weights of the complex \ac{GMM} are used as observations within a variational \ac{EM} approach for multi-source tracking that estimates as latent variables the source state, consisting of the source direction and velocity, as well as a latent assignment variable that associates each observation with a source state. New tracks are initiated from observations assigned to background noise and corresponding to a smooth trajectory over a short period of frames. The posterior \ac{pdf} of the assignment variables is used for multi-source \ac{VAD}.
  % \item [ID 7 \cite{Salvati2018a}] combines diagonal unloading beamforming \cite{Salvati2018} for localization with a Kalman filter for source tracking using a 7-microphone linear subarray of the \ac{DICIT} array for the single-source Tasks 1, 3 and 5. The \ac{CPSD} matrix is evaluated for the microphone signals in the \ac{STFT} domain. The trace of the \ac{CPSD} matrix is used as a \ac{VAD}. For voice-active frames, diagonal unloading is applied in order to attenuate the signal subspace by subtracting the \ac{CPSD} matrix and its trace. Instantaneous \ac{DoA} estimates in each time frame are obtained by broadband \ac{SRP} beamforming using the unloaded \ac{CPSD} matrix. A Kalman filter is applied to the \ac{DoA} estimates for source tracking.
  % \item [ID 8 \cite{Mosgaard2018}] combines \ac{TDE} with \acp{IPD} for localization and apply a wrapped Kalman filter \cite{Traa2013} for source tracking using the hearing aids in the single-source Tasks 1, 3 and 5. Circular statistics are exploited to obtain estimates of the \acp{IPD} and associated reliabilities. The \ac{IPD} estimates are mapped to \acp{TDoA} using a variance-weighted linear fit. The resulting \ac{TDoA} estimates are used to obtain estimates of the \ac{DoA}. A wrapped Kalman filter is applied to the \ac{DoA} estimates for source tracking.
  % \item [ID 10 \cite{Kitic2018}] combines localization using the first-order ambisonics configuration of the Eigenmike with a particle filter for single- and multi-source tracking for Tasks 1-4. A \ac{VAD} based on unbiased \ac{MMSE} noise power spectral estimates \cite{Gerkmann2012} is applied. For each voice-active period, the first-order ambisonic signals are computed as weighted scalar products between the microphone signals and the spherical harmonics. Pseudo-intensity vectors are evaluated from the \ac{STFT} of the first-order ambisonic channels. The \ac{DoA} estimates are extracted as the local maxima of the histograms of pseudo-intensity vectors, evaluated over observation intervals lasting 1~s. The \ac{DoA} estimates are used as observations within a particle filter for tracking the source positions. The importance weights correspond to a function of the angular distance between the \ac{DoA} estimates and the directions corresponding to the particle states. Hypothesis testing is applied for the association between \ac{DoA} estimates and tracks, and for the initialization of new tracks. Redundant tracks are removed by evaluating the angular distance between all pairs of track estimates. For each pair, the track corresponding to the shorter lifetime is penalized by reducing the associated importance weight.
  % \item [ID 13 \cite{Nakadai2018}] applies \ac{MUSIC} for localization and a Kalman filter for tracking the source \acp{DoA} for single-source Tasks 1 and 3 using the robot head and the Eigenmike. A \ac{VAD} based on zero-crossing rate and power thresholding is applied to each frame in the \ac{STFT} of the microphone signals. For each voice-active frame, \ac{MUSIC}, using the singular value decomposition for subspace analysis, is applied for \ac{DoA} estimation. The \ac{DoA} estimates are used as inputs to a Kalman filter in order to track multiple source directions. New tracks are initiated using unassociated \ac{DoA} estimates. Source termination is addressed using a preset parameter that indicates the duration during which a track was not associated with any \ac{DoA} estimates.
  % \item [ID 14 \cite{Nakadai2018}] extends the approach in ID 13 to use the \ac{GEVD} for the subspace decomposition in \ac{MUSIC}.
% \end{description}

% Approaches without \ac{VAD} (and hence no track latency):
% \begin{itemize}
%   \item Submissions 11 and 12, using \ac{DoA} estimation in the spherical harmonic domain
%   \item 6: Tracker
%   \item 1: {\color{red} Chase authors for details}
%   \item 5: Spherical harmonics Pavlini
%   \item 8: Wrapped KF
%   \item 2: Tracker?
%   \item 3: Tracker
%   \item 11 + 12
% \end{itemize}
% with \ac{VAD}:
% \begin{itemize}
%   \item 4: Tracker
%   \item 10: Tracker
%   \item 15 + 16: Doa estimation only
%   \item 13 + 14: MUSIC + KF
%   \item 7: DoA estimator
% \end{itemize}
% For 4, 7, 10, 13, 14, 15, 16: Provide delay between first detection (whether gated or not) and onset of VAD. For comparison to see if gating makes drastic difference!


==> Macros/latex.commands.miscellaneous.tex <==
% ============================================
% Commands for shortcuts to files.
% ============================================
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\etc}{\emph{etc.}}
\newcommand{\cf}{\emph{cf.}}
\newcommand{\etal}{\emph{et~al}.}
\newcommand{\role}{r\^{o}le}
\newcommand{\Bayes}{Bayes's}
\newcommand{\apriori}{\emph{\`{a} priori}\ }

% ==============================
% Commands for using in indexing
% ==============================

\newcommand{\bb}[1]{\textbf{#1}}
\newcommand{\ii}[1]{\textbf{#1}}
\newcommand{\zz}[1]{\textbf{#1}}
\newcommand{\nn}[1]{#1n}

\newcommand{\rv}{\mr}
\newcommand{\dv}{}

% \newcommand{\mydate}[3]{\begin{flushright} \Writinghand $\,$ \emph{Section created:} . \emph{Last revised:} #2 $#1^{th}, #3$. \end{flushright}}

==> Macros/latex.commands.symbols.tex <==
%!TEX root = /Users/cevers/Documents/Academic/PhDThesis/Reports/Thesis/ChristineEversMinutes.tex

% ==================================
% Commands for symbol defs
% ==================================

% general
\newcommand{\errorSignal}[1][t]{\ensuremath{\colvec{e}_{#1}}}
\newcommand{\ErrorSignal}[1][0:t]{\ensuremath{\colvec{e}_{#1}}}
\newcommand{\estimate}[1][t]{\ensuremath{\widehat{\colvec{x}}_{#1}}}
\newcommand{\Estimate}[1][0:t]{\ensuremath{\widehat{\colvec{x}}_{#1}}}
\newcommand{\sourceParam}[1][t]{\ensuremath{\colvec{a}_{#1}}}
\newcommand{\obserCovar}[1][t]{\ensuremath{\symvec{\phi}_{\colvec{w}_{#1}}}}
\newcommand{\processCovar}[1][t]{\ensuremath{\phi_{v_{#1}}}}
\newcommand{\processCovarMat}[1][t]{\ensuremath{\mat{\Sigma_{\colvec{v}_{#1}}}}}
\newcommand{\obserCovarMat}[1][t]{\ensuremath{\mat{\Sigma}_{w_{#1}}}}
\newcommand{\transitMat}[1][t]{\ensuremath{\mat{A}_{#1}}}
\newcommand{\param}[1][0:t]{\symvec{\theta}_{#1}}
\newcommand{\state}[1][t]{\colvec{x}_{#1}}
\newcommand{\State}[1][0:t]{\colvec{x}_{#1}}
\newcommand{\channel}{\colvec{b}}
\newcommand{\TVchannel}[1][t]{\channel_{#1}}
\newcommand{\prevObser}[1][t-1]{\colvec{y}_{#1}^T}
\newcommand{\obser}[1][t]{\colvec{y}_{#1}}
\newcommand{\Obser}[1][1:t]{\colvec{y}_{#1}}
\newcommand{\obserMat}[1][t-1]{\mat{Y}_{#1}}
\newcommand{\obserMatTV}[1][t-1]{\overline{\mat{Y}}_{#1}}
\newcommand{\kalmanGain}[1][t]{\mat{K}_{#1}}
\newcommand{\stateMat}[1][t]{\ensuremath{\mat{D}_{#1}}}
\newcommand{\stateCovar}[1][t]{\ensuremath{\mat{\Sigma}_{\mat{D}_{#1}}}}

% Kalman filter
\newcommand{\predMean}[1][t]{\symvec{\mu}_{#1|#1-1}}
\newcommand{\predCovar}[1][t]{\mat{\Sigma}_{#1|#1-1}}
\newcommand{\corrMean}[1][t]{\symvec{\mu}_{#1|#1}}
\newcommand{\corrCovar}[1][t]{\mat{\Sigma}_{#1|#1}}
\newcommand{\corrMeanPartAvg}[1][t]{\hat{\symvec{\mu}}_{#1|#1}}
\newcommand{\corrCovarPartAvg}[1][t]{\hat{\mat{\Sigma}}_{#1|#1}}
\newcommand{\obserResid}[1][t]{\ensuremath{z_{#1}}}
%\newcommand{\obserResidCovar}[1][t]{\ensuremath{\sigma_{z_{#1}}^2}}
\newcommand{\predError}[1][t]{\symvec{\epsilon}_{#1|#1-1}}
\newcommand{\corrError}[1][t]{\symvec{\epsilon}_{#1|#1}}
\newcommand{\corrMeanSource}[1][t]{\symvec{\mu}_{\colvec{x}_{#1|#1}}}
\newcommand{\predMeanSource}[1][t]{\symvec{\mu}_{\colvec{x}_{#1|#1-1}}}
\newcommand{\corrCovarSource}[1][t]{\mat{\Sigma}_{\colvec{x}_{#1|#1}}}
\newcommand{\predCovarSource}[1][t]{\mat{\Sigma}_{\colvec{x}_{#1|#1-1}}}
\newcommand{\sourceGain}[1][t]{\ensuremath{\mat{K}_{\colvec{x}_{#1}}}}
\newcommand{\crossCovarSourceChan}[1][t]{\ensuremath{\mat{\Sigma}_{(\colvec{x} | \colvec{b})_{#1}}}}
\newcommand{\crossCovarChanSource}[1][t]{\ensuremath{\mat{\Sigma}_{(\colvec{b} | \colvec{x})_{#1}}}}

% channel estimate
\newcommand{\chanMean}[1][t]{\symvec{\mu}_{\colvec{b}, #1}}
\newcommand{\chanCovar}[1][t]{\mat{\Sigma}_{\colvec{b}, #1}}
\newcommand{\residCovar}[1][t]{\ensuremath{\mat{\Sigma}_{z_{#1}}}}
\newcommand{\chanGain}[1][t]{\mat{K}_{\channel_{#1}}}
\newcommand{\chanResidCovar}[1][t]{\mat{\Sigma}_{\colvec{z}_{#1, \channel}}}

% marginalized estimated
\newcommand{\predMeanAlpha}[1][t]{\symvec{\alpha}_{#1|#1-1}}
\newcommand{\predMeanGamma}[1][t]{\mat{\Gamma}_{#1|#1-1}}
\newcommand{\corrMeanAlpha}[1][t]{\symvec{\alpha}_{#1|#1}}
\newcommand{\corrMeanGamma}[1][t]{\mat{\Gamma}_{#1|#1}}
\newcommand{\margMean}[1][t]{\hat{\symvec{\mu}}_{#1|#1}}
\newcommand{\margCovar}[1][t]{\hat{\mat{\Sigma}}_{#1|#1}}

\newcommand{\vars}[1][0:t]{\colvec{z}_{#1}}
\newcommand{\varsEst}[1][0:t]{\hat{\colvec{z}}_{#1}}
\newcommand{\allVars}[1][0:t]{\symvec{\varphi}_{#1}}
\newcommand{\allVarsEst}[1][0:t]{\hat{\symvec{\varphi}}_{#1}}
\newcommand{\exampleRV}[1][1]{\colvec{s}_{0:t, #1}}
\newcommand{\paramEst}[1][0:t]{\hat{\symvec{\theta}}_{#1}}
\newcommand{\stateEst}[1][t]{\hat{\colvec{x}}_{#1}}

\newcommand{\PFSFreq}[1][0:t]{\colvec{f}_{#1}}
\newcommand{\PFSBW}[1][0:t]{\colvec{B}_{#1}}
\newcommand{\PFSGain}[1][0:t]{\colvec{g}_{#1}}
\newcommand{\PARCOR}[1][0:t]{\symvec{\psi}_{#1}}

\newcommand{\gain}[1][]{\mat{G}_{#1}}
\newcommand{\gainVec}{\colvec{g}}

% MCMC case
\newcommand{\blockIndex}[1][i]{\ensuremath{\colvec{n}}}

==> Templates/IEEEtran/README <==

December 27, 2012


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

V1.8 is a significant update over the 1.7a release. For a full list of
changes, please read the file changelog.txt. The most notable changes
include:


 1) New transmag class option to support the IEEE Transactions on Magnetics
    format. Thanks to Wei Yingkang, Sangmin Suh and Benjamin Gaussens
    for suggestions and beta testing.

 2) The \IEEEcompsoctitleabstractindextext and 
    \IEEEdisplaynotcompsoctitleabstractindextext
    commands have been deprecated in favor of their
    \IEEEtitleabstractindextext and \IEEEdisplaynontitleabstractindextext
    (observe that the "not" has changed to "non") equivalents. This change
    generalizes and decouples them from compsoc mode because the new
    transmag mode also uses them now.

 3) Added new *-forms of \IEEEyesnumber*, \IEEEnonumber*, \IEEEyessubnumber*,
    and \IEEEnosubnumber* (the non-star form of the latter is also new) which
    persist across IEEEeqnarray lines until countermanded. To provide for
    continued subequations across instances of IEEEeqnarrays as well as for
    subequations that follow a main equation (e.g., 14, 14a, 14b ...)
    \IEEEyessubnumber no longer automatically increments the equation number
    on it's first invocation of a subequation group. Invoke both
    \IEEEyesnumber\IEEEyessubnumber together to start a new
    equation/subequation group.
 
 4) Hyperref links now work with IEEEeqnarray equations.
    Thanks to Stefan M. Moser for reporting this problem.

 5) Revised spacing at top of top figures and tables to better
    align with the top main text lines as IEEE does in its journals. 
    Thanks to Dirk Beyer for reporting this issue and beta testing.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> latex.preamble.IEEETran.tex <==
% Misc
\usepackage{amsfonts, amssymb, amsmath}	% Use math fonts
\usepackage{tabularx}					% For wrapping text in tables
\usepackage[table,usenames]{xcolor}
\usepackage{xfrac}
\usepackage{paralist}		% inline lists
\usepackage{breqn}			% break lines automatically in eqn.s
%\usepackage{algpseudocode}	% Pseudocode
\usepackage{pgfplots, tikz}
\usepackage{multicol}
\usepackage{enumitem}


% Definition for Matlab patch objects as legends in caption:
\usepackage{tcolorbox}
\newtcbox{\legendbox}[1][]{%
  nobeforeafter,
  colframe=black,
  boxrule=0.5pt,
  minipage,
  width=3ex,
  height=1.5ex,               %%% <--- change here
  arc=0pt,
  boxsep=0pt,
  #1
  }

% \setlength{\abovedisplayskip}{3pt}
% \setlength{\belowdisplayskip}{3pt plus 3pt minus 3pt}
% \setlength{\abovedisplayshortskip}{3pt}
% \setlength{\belowdisplayshortskip}{3pt plus 3pt minus 3pt}
%reduce space after figure captions
% \captionsetup[figure]{belowskip=-1.0em}
% \captionsetup[table]{position=above}

% Tikz plots:
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{backgrounds}
\pgfplotsset{compat=newest}
\pgfplotsset{
	every node/.style={font=\footnotesize},
  	every axis legend/.style={font=\footnotesize, fill=white, fill opacity=0.5},
  		x grid style={white},
	y grid style={white},
	% axis background/.style={fill=white!89.803921568627459!black}
  % axis background/.style={fill=white!89.803921568627459!black}
  	tick label style={font=\footnotesize},
  	ylabel style={font=\footnotesize, yshift=-0.5em},
  	xlabel style={font=\footnotesize, xshift=-0.5em},
  	yticklabel style={/pgf/number format/fixed},
  	xticklabel style={/pgf/number format/fixed},
  	/tikz/matlab2tikz picture/.append style={trim axis left, trim axis right},
  % every axis line/.append style={white},
  % every axis background/.append style={fill=black, fill opacity=0.3}
  	tick align=inside,
  	yminorticks=true,
  	xminorticks=true,
  	minor tick num={2},
  	max space between ticks=20pt,
}
%% the following commands are sometimes needed

% \pgfplotsset{%
%   every axis legend/.style={font=\footnotesize, fill opacity=0.8},
%   % axis background/.style={fill=white!89.803921568627459!black}
%   % tick label style={font=\footnotesize},
%   % ylabel style={font=\footnotesize, yshift=-0.5em},
%   % xlabel style={font=\footnotesize, xshift=-0.5em},
%   % yticklabel style={/pgf/number format/fixed},
%   % xticklabel style={/pgf/number format/fixed},
%   % /tikz/matlab2tikz picture/.append style={trim axis left, trim axis right}
%   % % every axis line/.append style={white},
%   % % every axis background/.append style={fill=black, fill opacity=0.3}
%   % tick align=outside,
%   % yminorticks=true,
%   % xminorticks=true,
%   % minor tick num={2},
%   % max space between ticks=20pt,
% }
\pgfplotsset{contourstyle/.style={%
  	x grid style={gray},
		y grid style={gray},
    width=\columnwidth,
	  % xtick={0,2,...,8},
	  % ytick={0,2,...,10},
	  minor y tick num={1},
	  minor x tick num={1},
	  yminorticks=true,
	  xminorticks=true,
	  fill opacity=0.6,
	  grid = both,
	  }}

  \pgfplotsset{barstyle/.style={%
        width=\columnwidth,
  	  ytick={0,0.1,...,2},
  	  minor y tick num={1},
  	  minor x tick num={1},
  	  yminorticks=true,
  	  xminorticks=true,
  	  fill opacity=0.6,
  	  grid = both,
  	  }}

\pgfplotsset{ colorbar style/.code={}, every colorbar/.append style={ /pgf/number format/fixed, ytick={0,0.2,...,1.01}, at={(1.05,1)} }}

\newlength\figheight
\newlength\figwidth

% Acronyms
\usepackage[printonlyused,withpage]{acronym}
%\usepackage[printonlyused]{acronym}
\newcommand{\acronymlist}[1]{
\begin{acronym}[MMMMMMM]\input{#1}\end{acronym}}
\newcommand{\acronymnolist}[1]{
\newcommand{\acro}{\acrodef}\newcommand{\acroindefinite}{\acrodefindefinite}\input{#1}}

% Nomenclature
\usepackage{letltxmacro}
\LetLtxMacro{\oldnomenclature}{\nomenclature}
\usepackage{ifthen}
\providecommand{\nomenclature}{}
\renewcommand{\nomenclature}[3][a]{\ifthenelse
  {\equal{#3}{ }}{\ac{#2}}{\ifthenelse
  {\equal{#3}{f}}{\acf{#2}}{\ifthenelse
  {\equal{#3}{s}}{\acs{#2}}{\ifthenelse
  {\equal{#3}{l}}{\acl{#2}}{\ifthenelse
  {\equal{#3}{p}}{\acp{#2}}{\ifthenelse
  {\equal{#3}{fp}}{\acfp{#2}}{\ifthenelse
  {\equal{#3}{sp}}{\acsp{#2}}{\ifthenelse
  {\equal{#3}{lp}}{\aclp{#2}}{\ifthenelse
  {\equal{#3}{fi}}{\acfi{#2}}{\ifthenelse
  {\equal{#3}{u}}{\acused{#2}}{\ifthenelse
  {\equal{#3}{su}}{\acsu{#2}}{\ifthenelse
  {\equal{#3}{lu}}{\aclu{#2}}{\ifthenelse
  {\equal{#3}{i}}{\iac{#2}}{\ifthenelse
  {\equal{#3}{I}}{\Iac{#2}}{\oldnomenclature[#1]{#2}{#3}}}}}}}}}}}}}}}}

% Macros
\input{/Users/cevers/Dropbox/Work/LaTeX/Macros/latex.commands.referencing}
\input{/Users/cevers/Dropbox/Work/LaTeX/Macros/latex.commands.equations.tex}
\input{/Users/cevers/Dropbox/Work/LaTeX/Macros/latex.commands.equations.stats.tex}

